Proposal to upgrade the MIPP Experiment

The upgraded MIPP physics results are needed for the support of NuMI projects, atmospheric cosmic ray and neutrino programs worldwide and will permit a systematic study of non-perturbative QCD interctions. The MIPP TPC is the largest contributor to the MIPP event size by far. Its readout system and electronics were designed in the 1990's and limit it to a readout rate of 60 Hz in simple events and ~20 Hz in complicated events. With the readout chips designed for the ALICE collaboration at the LHC, we propose a low cost scheme of upgrading the MIPP data acquisition speed to 3000 Hz. This will also enable us to measure the medium energy numi target to be used for the NOvA/MINERvA experiments. We outline the capabilities of the upgraded MIPP detector to obtain high statistics particle production data on a number of nuclei that will help towards the understanding and simulation of hadronic showers in matter. Measurements of nitrogen cross sections will permit a better understanding of cosmic ray shower systematics in the atmosphere. In addition, we explore the possibilities of providing tagged neutral beams using the MIPP spectrometer that may be crucial for validating the Particle Flow Algorithm proposed for calorimeters for the International Linear Collider detectors. Lastly, we outline the physics potential of such a detector in understanding non-perturbative QCD processes.

==> offline_impact.tex <==
\section{Offline resources needed}


==> upgr_new_physics.tex <==
\section{Additional Physics that can be done with the upgraded MIPP}

In addition to the physics approved for MIPP I (acquirable in under 20 days), 
the upgrade 
extends MIPP's physics capabilities considerably  in the following sectors.




\subsection{Low momentum pion and kaon physics}

We have run the MIPP secondary beam line between the momenta 75 GeV/c
to 5 GeV/c. The beam line power supplies regulate well down to 5
GeV/c but cannot accurately be controlled below this at present, because
the currents become too small. However, we can use trim dipole power
supplies (plentiful at Fermilab) below 5 GeV/c~\cite{lenz} and control the beam line
well. MIPP would then switch between the two sets of supplies,
depending on beam conditions.  We can identify the particles in the
beam well using our beam Cerenkovs and time of flight. The time of
flight will be used for low energy beams. The beam fluxes at our secondary target, 
taking into account decay in flight, are given in table~\ref{lowbeam}.

\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c||c|c|c|} 
\hline
Momentum   & p	& $K^+$ & $\pi^+$ & $\bar{p}$ & $K^-$ & $\pi^-$ \\
GeV/c      &    &       &         &         &       &       \\
\hline
\hline
1  &  5752  &  0  &  64798  & 7907  &  0  &  30425 \\
2  &  23373  &  194  &  459718  & 26863  &  142  &  236494 \\
3  &  53431  &  3060  &  1069523 & 51424  &  2221  &  598742 \\
5  &  153220  &  32763  &  2400799  & 103996  &  23164  &  1550810 \\
10  &  663916  &  223210  &  5006708  &  195767  &  142777  &  3862225 \\
15  &  1618120  &  443557  &  7141481  & 221602  &  245868  &  5248463 \\
20  &  3113387  &  655426  &  9290219  & 212171  &  306685  &  5841030 \\
30  &  8158054  &  1043430  &  12770579  & 160329  &  340144  &  5837467 \\
40  &  16664431  &  1294189  &  13944272  & 101617  &  288728  &  5156862 \\
50  &  29288928  &  1338452  &  12788523  &  53056  &  196400  &  4114582 \\
60  &  45985629  &  1191744  &  10094311  &  22092  &  108032  &  2905091 \\
70  &  65227010  &  919279  &  6834097  &  6987  &  47093  &  1762060 \\
\hline
\hline
\end{tabular}
\caption{Secondary beam fluxes as a function of beam momentum and species for 2E11 primary protons on target~\label{lowbeam}}
\end{center}
\end{table}
 The present distance from the primary to the secondary target is 95
 meters. With no change in beam line design, it is possible to produce
 a 1 GeV/c pion beam and kaon beams down to 5 GeV/c. With the high DAQ
 rate of the upgraded MIPP, this permits searches for missing baryon
 resonances. It also permits us to search for exotic resonances such as
 pentaquarks or glueballs using six beam species and varying beam
 momenta. These abilities would make MIPP unique in this field. It can
 complement the results of photon beam searches at places such as the
 Jefferson Laboratory (Jlab).

